Pacos: Modeling Users' Interpretable and Context-Dependent Choices in Preference Reversals

Choice problems refer to selecting the best choices from several items, and learning users' preferences in choice problems is of great significance in understanding the decision making mechanisms and providing personalized services. Existing works typically assume that people evaluate items independently. In practice, however, users' preferences depend on the market in which items are placed, which is known as context effects; and the order of users' preferences for two items may even be reversed, which is referred to preference reversals. In this work, we identify three factors contributing to context effects: users' adaptive weights, the inter-item comparison, and display positions. We propose a context-dependent preference model named Pacos as a unified framework for addressing three factors simultaneously, and consider two design methods including an additive method with high interpretability and an ANN-based method with high accuracy. We study the conditions for preference reversals to occur and provide an theoretical proof of the effectiveness of Pacos in addressing preference reversals. Experimental results show that the proposed method has better performance than prior works in predicting users' choices, and has great interpretability to help understand the cause of preference reversals.

==> data/MNL.tex <==
\section{The proposed framework}
\label{sec:framework}
We briefly review the framework of discrete choice models, which is the background of our proposed model. Discrete choice models contains a class of models which is designed for discrete choice problems, such as multinomial logit model (MNL), nested logit model, and random coefficient model. Among the above models, as MNL is simplest and has good interpretability, it is the most widely used model in real applications.

As discussed in Section \ref{sec:intro}, in a discrete choice problem setting, a user faces several available items, and is required to select the most preferred item. In this work, we use $\mathcal{S}$ to denote the choice set and $\boldsymbol{s_i}$ the $i$-th item, that is, $\mathcal{S}=\{\boldsymbol{s}_i\}$, where $i=1,\cdots,N$ and $N$ is the number of items. Each item $\boldsymbol{s_i}$ is described by a vector of $d$ attributes, i.e., $\boldsymbol{s_i}\in\mathbb{R}^d$. Let the most preferred item be $\boldsymbol{s_b}$, then the discrete choice dataset is a set of pairs $\{(\boldsymbol{s_b},\mathcal{S})\}$.

In MNL, \emph{utility} is used to quantify a user's satisfactory level for an item, and a larger utility value indicates the user's higher preference. We assume the user is rational and always choose the item with the largest utility value. Let $U(\boldsymbol{s}_i)$ be the user's utility for item $\boldsymbol{s}_i$. In MNL, $U(\boldsymbol{s}_i)$ is decomposed into two parts, that is,
\begin{align}
U(\boldsymbol{s}_i) = V(\boldsymbol{s}_i)+\epsilon{(\boldsymbol{s}_i)}
=\boldsymbol\beta^T\boldsymbol{s}_i+\epsilon{(\boldsymbol{s}_i)},
\end{align}
where $V(\boldsymbol{s}_i)$ is the intrinsic value that is determined by the item's attributes, and $\epsilon_{\boldsymbol{s}_i}$ is the error term that captures noise and other unobserved factors. In detail, for $V(\boldsymbol{s}_i)$, it is assumed to be the weighted sum of the item's attributes, and the vector $\boldsymbol\beta$ stores the user's weight or relative importance for each attribute. For the error term $\epsilon{(\boldsymbol{s}_i)}$, it is considered to be a random variable, and follows the type I extreme value distribution with the probability density function being $f(\epsilon)=e^{-\frac{\epsilon-\mu}{\sigma}}e^{-e^{-\frac{\epsilon-\mu}{\sigma}}}$ and cumulative distribution function being $F(\epsilon)=e^{-e^{-\frac{\epsilon-\mu}{\sigma}}}$, where $\mu$ is the location parameter and $\sigma$ is the scale parameter, which are related to the mean and standard deviation of $\epsilon$, respectively. Generally, we $\mu=0$ and $\sigma=1$, and $\epsilon$ is independent and identically distributed for all items in the choice set. Under the above settings, the probability that an item $\boldsymbol{s}_i$ is selected by the user can be written as
\begin{align}
P(\boldsymbol{s}_i)=P\left(U(\boldsymbol{s}_i)\geq U(\boldsymbol{s}_j),\forall i\neq j\right)
=\frac{\exp{(\boldsymbol\beta^T\boldsymbol{s}_i)}}{\sum_{j=1}^{N}\exp{(\boldsymbol\beta^T\boldsymbol{s}_i)}}.
\end{align}
the relationship with the softmax function used in machine learning field.

Although MNL is simple and applied in many studies, it suffers from the \emph{independence of irrelevant alternatives (IIA)} assumption, which limits its accuracy performance in practice. The IIA assumption states that the ratio of selected probabilities of any two items is not affected by a third item. Formally, we have
\begin{align}
\frac{P(\boldsymbol{s}_i)}{P(\boldsymbol{s}_j)}=\frac{\exp{(\boldsymbol\beta^T\boldsymbol{s}_i)}}{\exp{(\boldsymbol\beta^T\boldsymbol{s}_j)}},
\end{align}
which is not affected by other items in the choice set. The IIA assumption is often violated in real applications, for example, the three context effects discussed in Section \ref{sec:intro}. That is to say, MNL cannot address the three context effects theoretically.

Nested logit model and mixed logit model are both extensions of MNL. To model the correlations among items, nested logit model partitions the choice set into several ``nests'', and items in a same nest have some similar attributes. Nested logit model is able to address the similarity effect. While to capture the taste variance in populations, mixed logit model divides all users into several segments, and users in a same segment is assumed to have similar preference. Mixed logit model is effective for the similarity effect and compromise effect. Both of the two models can only explain a part of the three context effects.





==> data/strategy.tex <==
\section{Optimal Pricing Strategy}
\label{sec:strategy}

\subsection{User Performance}

\subsubsection{One User}

According to the previous chapter, the user's personal weight $\alpha_{u}$ is assumed to be uniformly distributed in the range.
\begin{equation}
    \alpha_{u} \sim
    U(\underline\alpha_{u}, \overline\alpha_{u})
\end{equation}

\subsubsection{Multiple Users}

For a large collection of users, we can estimate the range of each user's $\alpha$, and then superimposed as the overall market preference distribution.

Define $F(\alpha)$ as the probability distribution function of the user preference parameter $\alpha$, which is obtained by  analyzing the purchase records of all or most consumers in the market in the past period of time. 
Considering $ 0\leq \alpha \leq 1$, there are $F(0) = 0$ and $F(1) = 1$. 
Similarly, we define $f(\alpha)$ as the probability density function.
\begin{equation}
    \label{equ:users-prob}
    \mathcal{P}_i = 
    \mathcal{P}[s_i = best | S] = 
    F(\bar{\alpha}_{i}) - F(\underline{\alpha}_{i}) = 
    \int_{\underline{\alpha}_{i}}^{\bar{\alpha}_{i}}{f(\alpha)d\alpha}
\end{equation}

\subsection{Commercial Competition}

Based on the previous model, we then analyze the calculation of the upper and lower bounds of the global variable $\alpha$ in the competitive market.

\subsubsection{Convex Set}

Each item is projected to point $(p, r)$ based on the normalized pricing and reputation, and then to the logarithmic coordinate plane, ie $(\ln{p}, \ln{r})$.
On the logarithmic plane, $\ln{r}$ decreases as $\ln{p}$ increases, as shown in Fig.\ref{fig:competitor}(a).
Define the market convex area as the convex area around all item points and the lower left region.
Set the vertices of the convex area of the market from left to right followed by $S_1, S_2, \cdots, S_{n}$, which constitute the market convex set, . We study the convex set and have the Lemma and Theorem 1.

Define $k = \displaystyle\frac{- \alpha}{1-\alpha} \leq 0$ , and $k_{S_i,S_j}$ or $k_{i,j}(i<j)$ as the slope of point $S_i$ and $S_j$ in the logarithmic plane.

\textbf{Lemma}: Under the condition of $i<j$, $U_i \leq U_j$ when $k \leq k_{i,j} < 0$, and  $U_i > U_j$ when $k_{i,j} < k < 0$.

\textbf{Proof of lemma}:
\[
    \begin{aligned}
    U_j - U_i &= \alpha (\ln{p_j} - \ln{p_i}) + (1-\alpha) (\ln{r_j}-\ln{r_i}) \\
    &= (\ln{p_j} - \ln{p_i})(\alpha + (1-\alpha) \frac{\ln{r_j}-\ln{r_i}}{\ln{p_j} - \ln{p_i}}) \\
    &= (\ln{p_j} - \ln{p_i})(\alpha + (1-\alpha) k_{i,j}) \\
    &= (\ln{p_j} - \ln{p_i})(1-\alpha)(k_{i,j}-k)
    \end{aligned}
\]
where $\ln{p_j} - \ln{p_i} > 0 ~(i<j)$ and $1-\alpha \geq 0$. So $U_i \leq U_j$ when $k \leq k_{i,j} < 0$, and  $U_i > U_j$ when $k_{i,j} < k < 0$.

\textbf{Theorem 1}: The point or item $S^*$ which is inside the convex hull would not be selected by the consumer group.

\textbf{Proof of Theorem 1}: Suppose point $S^*(p^*,r^*)$ is near two vertices $S_i,S_{i+1}$ and $p_i < p^* < p_{i+1},~ r_i > r^* > r_{i+1}$.

Let the linear equation through $S_i$ and $S_{i+1}$ be $(\ln{r}) - k_{i,i+1} (\ln{p}) + C = 0$, where $C$ is a constant number. As the point $S^*(p^*,r^*)$ is under the line $S_i S_{i+1}$, we have $(\ln{r^*}) - k_{i,i+1} (\ln{p^*}) + C < 0$, then
\[
    \ln{r^*} - \ln{r_i}  < k_{S_{i},S_{i+1}}(\ln{p^*} - \ln{p_i})
\]
Combine with
\[
 \ln{r^*} - \ln{r_i}  = k_{S_{i},S*}(\ln{p^*} - \ln{p_i})
\]
then
\[
    (k_{S_{i},S^*} - k_{S_{i},S_{i+1}})(\ln{p^*} - \ln{p_i}) < 0
\]
which means that $k_{S_{i},S^*} < k_{S_i,S_{i+1}}$.
Similarly, $k_{S_i,S_{i+1}} < k_{S^*,S_{i+1}}$.

We can get that $k_{S_{i},S^*} < k_{S_i,S_{i+1}} < k_{S^*,S_{i+1}}$. 
For any consumer in the group with the corresponding global parameter equals $k$. When $k \leq k_{i,i+1}$, $k \leq k_{i,i+1} < k_{S^*,S_{i+1}}$, then $U_{S^*} < U_{i+1}$ according to the Lemma. Similarly, $U_{S^*} < U_{i}$ when $k > k_{i,i+1}$. 

So $S^*$ would not be selected by the rational consumer group. Theorem 1 has been proved.

\begin{figure}
    \begin{minipage}{0.49\linewidth}
    \centerline{\includegraphics[width=0.8\linewidth]{convex-1.jpg}}
    \centerline{(a) Convex Set}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\linewidth}
    \centerline{\includegraphics[width=0.8\linewidth]{convex-2.jpg}}
    \centerline{(b) Price Interval}
    \end{minipage}
    \caption{Pricing Strategy}
    \label{fig:competitor}
\end{figure}  

\subsubsection{Competitors}

The upper and lower limits of the $\alpha_i$ are determined by seller's key competitors. 
Through the study of the competitive situation, we get

\textbf{Theorem 2}: The key competitors of $S_i$ are the adjacent vertices. The range of $k$ that can be attracted by the vertex $S_i$ is $(k_{i, i + 1}, k_{i-1, i}), ~ 1<i<n$.

\textbf{Proof of Theorem 2}: Firstly, we prove the necessity of the range $(k_{i, i + 1}, k_{i-1, i})$, which means that if $S_i$ was attracted, the slope $k \in (k_{i, i + 1}, k_{i-1, i})$. Then we prove when $k \in (k_{i, i + 1}, k_{i-1, i})$, the utility of $S_i$ would be the largest one.

Necessity: As $U_i$ is the largest value of utility, then $U_i > U_{i+1}$ and $U_i > U_{i-1}$, which means $k > k_{i,i+1}$ and $k < k_{i-1,i}$, so $k \in (k_{i, i + 1}, k_{i-1, i})$.

Sufficiency: When $k > k_{i,i+1}$, since $ S_{i}S_{i +1} $ is the boundary of the convex region, similar to the analysis in the Theorem 1, we have $k_{i,l} \leq k_{i,i+1}$, $l \geq i+1$, so $U_i > U_l$,$l \geq i+1$. Similarly, $U_i > U_u$, $u \leq i-1$ when $k < k_{i-1,i}$. So $U_i$ is the greatest utility.

In summary, Theorem 2 is proved.

\textbf{Inference}: $k \in (k_{i,i+1},k_{i-1,i})$ corresponds the global parameter $\alpha \in (\underline{\alpha}_{i}, \bar{\alpha}_{i})$. The $S_i$ is the best choice if and only if $\alpha \in (\underline{\alpha}_{i}, \bar{\alpha}_{i})$.

\subsection{Pricing Algorithm}

Firstly, we simplify the optimization goal mentioned in the opening section.
\begin{equation}
\label{equ:aim-simply}
        \max_{0 \leq p_i \leq 1}{(C - p_i)(F(\bar{\alpha}_{i}) - F(\underline{\alpha}_{i}))}
\end{equation}

When $p_i$ increases, the market convex set and the key competitors of $s_i$ may change correspondingly, so we need to find the interval of $p_i$ where the key competitors remains the same.

In this subsection, we propose the Optimal Pricing Strategy. Firstly, get the convex set obtained by all sellers except $s_i$ by \textbf{Algorithm \ref{alg1}}.

\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}
    \caption{Get the convex set}   
    \label{alg1}  
    \begin{algorithmic}[1]
    \REQUIRE  Items with $r_1 < r_2 < \cdots < r_N$
    \ENSURE  Vertices $V=\{S_1, S_2, \cdots, S_{n}\}$
    \STATE Remove $s_i$ from item set and renew the subscripts
    \STATE add $S_1$ to $V$ and $index \Leftarrow 1$
    \WHILE{$index < N-1$}
    \STATE Define $k_n = (\ln{r_n}-\ln{r_{index}})/(\ln{p_n}-\ln{{p_{index}}})$
    \STATE $k_j \Leftarrow \max_{index<n<N}{k_n}$
    \STATE add $S_j$ to $V$ and $index \Leftarrow j$
    \ENDWHILE 
    \end{algorithmic}  
\end{algorithm}  

Afterwards, as shown in Fig.{\ref{fig:competitor}(b)}, sort the intersection points of each line of two adjacent vertices and the fixed line $r = r_i$, and find out the key competitors when $p_i$ in each interval between two intersections by \textbf{Algorithm \ref{alg2}}. For example, when $p_2<p_i<p_3$ shown in Fig.{\ref{fig:competitor}(b)}, the key competitors of seller $I$ would be seller $B$ and $D$.

\begin{algorithm}
    \caption{Find out the key competitors}   
    \label{alg2}  
    \begin{algorithmic}[1]
    \REQUIRE Vertices $V=\{S_1, S_2, \cdots, S_{n}\}$ and $r_i$
    \ENSURE Dictionary \{$p,S_u,S_l$\} where $p$ means the lower of interval and $S_u,S_l$ are the corresponding competitors
    \STATE Calculate the intersection of line $S_jS_{j+1}(1\leq j <n)$ 
    and the fixed line $\ln{r} = \ln{r_i}$ and get the intersection tuple $\{p_j , S_{j^*_1}, S_{j^*_2}\}$ where $j^*_2 = j^*_1 + 1$
    \STATE Sort the tuple by $p$ from small to large
    \STATE Initialize the result dictionary to the tuple
    \IF{$r_{S_1} < r_i < r_{S_n}$}
        \STATE $index \Leftarrow 1$
        \WHILE{$index < n$}
            \IF{$S_{{(index-1)}^*_2}= S_{{index}^*_1}$}
                \STATE $S_{{index}^*_1} \Leftarrow S_{{(index-1)}^*_1}$  
            \ENDIF
            \IF{$S_{{(index-1)}^*_1} = S_{{index}^*_2}$}
                \STATE $S_{{index}^*_2} \Leftarrow S_{{(index-1)}^*_2}$
            \ENDIF
        \ENDWHILE
    \ELSE
        \STATE Update the tuple similarly
    \ENDIF
    \end{algorithmic}  
\end{algorithm}  

Then, we use the history records of users to get the $\alpha$'s probability distribution function $F(\alpha)$ and calculate the optimal price in each interval of $p_i$ by implicit enumeration method or other optimization algorithms. Lastly, we integrate all the optimums to get the best global pricing.

==> data/train.tex <==
\section{The Training Procedure}
\label{sec:train}
In the previous section, we have discussed the utility function and propose two calculation methods. The next question is how to learn parameters in the utility function when given the user's transaction records, which is the focus of this section. For the additive method in Fig. \ref{fig:g_and_h}, parameters that need to be learnt include the two multiplier matrices in $g(\cdot)$, two multiplier matrices in $h(\cdot)$, and the user's preference for display position $\boldsymbol\alpha$. Similarly, for the ANN-based method in Fig. \ref{fig:G_and_H},  we should learn parameters of the neural networks in $G(\cdot)$ and $H(\cdot)$, respectively, and $\boldsymbol\alpha$ as well. Although the two methods need to learn different parameters, the proposed training procedure can be applied to both methods.

Based on the model overview in Fig. \ref{fig:overall_structure}, the part denoted by green is the proposed training procedure, which includes three components, that is, a loss function that need to be optimized, an utility bar $\bar B$ that is used to avoid partial-training issue, and an update rule that adjusts the value of $\bar B$ flexibly in the training process. The pseudocode of the training procedure is provided in Algorithm \ref{algo:training}. In the following, we explain the three components in details.

First, we use the cross entropy \cite{de2005tutorial}
\begin{align}
\label{equ:loss}
  l = -\sum_{t=1}^T\sum_{i=1}^N y_i\log \mathcal{P}(\boldsymbol s_i|\mathcal{S}),
\end{align}
as the loss function, where $\mathcal{P}(\boldsymbol s_i|\mathcal{S})$ is the probability of being selected in Eq. (\ref{equ:prob_new}),  and $y_i$ is an indicator with $y_i=1$ if $\boldsymbol s_i$ is the user's selected item and $y_i=0$ otherwise. The training procedure optimizes the above parameters so that the total loss on transaction records is minimized.

Note that the partial-training issue may occur in the training procedure. Consider the scenario that all markets contain four items, which are sorted by the ascending order of their reputations, and the user always selects items that displayed at the forth rank. In this case, the training procedure may quickly find a solution, that is, the forth element in the user's preference for position $\boldsymbol\alpha$ is a high value, and other parameters of $g(\cdot)$ and $h(\cdot)$ in the additive method, or $G(\cdot)$ and $H(\cdot)$ in the ANN-based method, are all zero. This solution can perfectly fit the phenomenon that the user always selects the forth-rank items in records. However, the user's selection of these items perhaps is not due to their displayed positions. For example, it is possible that the user just wants to select an item with the highest reputation, and all of the selected items have the largest reputations and are displayed at the forth rank at the same time. In such a case, the above found solution overestimates the user's preference for display position, while underestimates or neglects his/her priority for reputation. When facing a new market with five items, the user selects the fifth item as it has the largest reputation. However, the found solution still regards the forth item as the best choice and outputs false prediction. Similarly, sometimes the training procedure may exaggerate the interaction among items and neglect the user's tradeoff among attributes. In this work, the phenomenon that the training procedure pays too much attention to one part of utility while neglects others is defined the partial-training issue. This issue could be solved by collecting the user's more transaction records. For example, if the record that the user selects the fifth item is in the training dataset, the training procedure may notice that the user's focus is the reputation rather than the display position, then optimize the parameters in attribute utility module further. However, on the individual level, the user's transaction records are usually limited, thus collecting more records to address the partial-training issue is not practical in reality.

In this work, to avoid the partial-overfitting issue, we introduce a variable, the bar of utility $\bar B$, into the training procedure, such that
\begin{align}
\label{equ:bar}
IU(\boldsymbol s_i|\mathcal{S}) = \min\{IU(\boldsymbol s_i|\mathcal{S}),\bar B\}, \quad \text{and}\quad PU(\boldsymbol s_i|\mathcal{S})=\min\{PU(\boldsymbol s_i|\mathcal{S}),\bar B\}.
\end{align}
In this way, if the training procedure originally pays too much attention to the interaction utility or the position utility, then $\bar B$ serves as the maximum value that the two parts can contribute to the total utility, then the training procedure is forced to optimize the user's tradeoff among attributes further and the partial-training problem is alleviated.

Considering the value of $\bar B$ may affect the model's performance, to avoid the inconvenience of manual selection of $\bar B$, we propose a novel update rule to dynamically adjust its value in the training procedure, that is,
\begin{align}
\label{equ:update}
\bar B = \min\left\{\left\lfloor\frac{k-K_{init}}{\Delta K}\right\rfloor\cdot \Delta B, B_{max}\right\}.
\end{align}
In Eq. (\ref{equ:update}), $k$ is the current epoch during training, and $B_{max}$ is the maximum value of $\bar B$. At the first $K_{init}$ epochs, $\bar B$ is initialized as 0. Then, after every $\Delta K$ epochs, $\bar B$ increases its value by $\Delta B$ until it reaches $B_{max}$. The $K_{init}$, $\Delta K$, $\bar B$, and $B_{max}$ are hyperparameters, and the impact of parameter selection on the performance is shown in Section \ref{sec:test}. The update rule forces the training procedure to focus on the user's tradeoff at the first $K_{init}$ epochs, and parameters in the interaction utility module and position module are optimized gradually during subsequent training epochs, which can alleviates the partial-training issue to some extent.

\begin{algorithm}[!t]
  \caption{The Training Procedure}
  \begin{algorithmic}[1]
  \Require $T$ records
  \Ensure The trained model
  \State Initialize parameters
  \For{$k=1$ to $K$}
  \If{$k<K_{init}$}
  \State $\bar B=0$
  \Else
  \State Compute $\bar B$ according to Eq. (\ref{equ:update})
  \EndIf
  \State Obtain $AU(\boldsymbol s_i)$, $IU(\boldsymbol s_i)$, and $PU(\boldsymbol s_i)$ according to Eq. (\ref{equ:uti_add}) or (\ref{equ:uti_nn})
  \State Refine $IU(\boldsymbol s_i)$ and $PU(\boldsymbol s_i)$ according to Eq. (\ref{equ:bar})
  \State Get $\mathcal{P}(\boldsymbol s_i)$ according to Eq. (\ref{equ:prob_new})
  \State Calculate the current loss $l$ according to Eq. (\ref{equ:loss})
  \State Update parameters that need to be trained through optimizer
  \EndFor
  \end{algorithmic}
   \label{algo:training}
\end{algorithm}

%After the training procedure, we obtain the optimized choice model that has learnt the user's preference. Given a new market with several items, the trained choice model is used to estimate each item's probability of being selected. The probability is very useful in real applications. For example, these items can be sorted in a descending order of their probabilities to generate a recommendation list for users.   Besides, on the market level,  adding up the probability of choosing an item along all users, also provides a good estimator of the item's market share in the new market. 
